Vistaar: Diverse Benchmarks and Training Sets for Indian Language ASR

Improving ASR systems is necessary to make new LLM-based use-cases accessible to people across the globe. In this paper, we focus on Indian languages, and make the case that diverse benchmarks are required to evaluate and improve ASR systems for Indian languages. To address this, we collate Vistaar as a set of 59 benchmarks across various language and domain combinations, on which we evaluate 3 publicly available ASR systems and 2 commercial systems. We also train IndicWhisper models by fine-tuning the Whisper models on publicly available training datasets across 12 Indian languages totalling to 10.7K hours. We show that IndicWhisper significantly improves on considered ASR systems on the Vistaar benchmark. Indeed, IndicWhisper has the lowest WER in 39 out of the 59 benchmarks, with an average reduction of 4.1 WER. We open-source all datasets, code and models.

==> styles.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% File:     INTERSPEECH2023.cls % class file for INTERSPEECH2023
%
% Usage:    \documentclass{INTERSPEECH2023}
%
% Purpose:
%
% Style file for INTERSPEECH 2023 Conference.
% Modified from previous INTERSPEECH conferences
% Features:
%    - correct page size (175mm x 226mm)
%    - use Times-Roman font as default font (roman font) in order to achieve
%      best quality on paper and screen
%    - two-column format
%    - boldfaced, numbered, and centered section headings
%    - correct subsection and subsubsection headings
%    - \sloppy is now the default but can be changed to \fussy by
%      specifying it as a package option (i.e. \usepackage[fussy]{INTERSPEECH})
%    - use \title{xx} for title, will be typeset all uppercase
%    - use \name{xx} for author name(s) only, will be typeset in italics
%    - use \address{xx} for authors' affiliations, one per line
%    - use \email{xx} for authors' email addresses, will be typeset
%      in proportional typeface
%    - note: no need for \author nor \date
%    - optional: can use \thanks{xx} within \name, asterisk is
%      not printed after name nor in footnote
%    - optional: can use \sthanks{xx} after each name within \name,
%      footnote symbol will appear for each name and footnote
%
%
% PLEASE REPORT ANY BUGS to Simon.King@ed.ac.uk
%
% Author:  Stephen Martucci  -- martucci@cdg.nj.nec.com
% Modifications: Jyri Huopaniemi -- jyri.huopaniemi@nokia.com
%                Matti Karjalainen -- matti.karjalainen@hut.fi
%                Panayiotis Georgiou -- panayiotis.georgiou@gmail.com
%                Mattias Heldner -- heldner@ling.su.se
%                Marcin W??odarczak -- wlodarczak@ling.su.se
%                Prasanta Ghosh -- prasantag@gmail.com
%                Simon King -- Simon.King@ed.ac.uk
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{INTERSPEECH2023}[2023/01/06 Official Interspeech 2023 package]

\LoadClass[a4paper]{article}

\RequirePackage{graphicx}
\RequirePackage{amssymb,amsmath,bm}
\RequirePackage{textcomp}
\RequirePackage{booktabs}
\RequirePackage[textfont=it,tableposition=top]{caption}
\RequirePackage{siunitx}
\RequirePackage{xspace}
\RequirePackage{url}
\RequirePackage{lipsum}  
\RequirePackage{tipa}
\RequirePackage{enumitem}

% hyperref is used to ensure author names 
% do not appear in PDF metadata
\RequirePackage[pdfauthor={Author name(s) withheld},
                pdftitle={Submitted to INTERSPEECH},
                colorlinks=false,
               ]{hyperref}

% but we also tell hyperref to disable hyperlinks
\AtBeginDocument{\NoHyper}

% reasonably compact lists
\AtBeginDocument{\setlist{noitemsep,topsep=2pt,parsep=2pt,partopsep=0pt,leftmargin=1em}}

\newif\ifinterspeechfinal
\interspeechfinalfalse
\def\interspeechcameraready{\global\interspeechfinaltrue}


\newif\if@fussy
\DeclareOption{fussy}{%
  \@fussytrue
}
\DeclareOption*{\OptionNotUsed}
\ProcessOptions\relax

\if@fussy
  \fussy
\else
  \sloppy
\fi

\def\vec#1{\ensuremath{\bm{{#1}}}}
\def\mat#1{\vec{#1}}



%change default font to Times-Roman
\renewcommand{\sfdefault}{phv}
\renewcommand{\rmdefault}{ptm}
\renewcommand{\ttdefault}{pcr}

\renewcommand{\section}{\@startsection
  {section}%
  {1}%
  {}%
  {-\baselineskip}%
  {0.5\baselineskip}%
  {}}%

\renewcommand{\subsection}{\@startsection
  {subsection}%
  {2}%
  {}%
  {-\baselineskip}%
  {0.5\baselineskip}%
  {}}%

\renewcommand{\subsubsection}{\@startsection
  {subsubsection}%
  {3}%
  {}%
  {-\baselineskip}%
  {0.5\baselineskip}%
  {}}%

%% these are the A4 settings
\oddsidemargin -0.20in % -0.31in
\evensidemargin -0.20in % -0.31in
\topmargin 0truept
\headheight 0truept
\footskip 0truept % 0truept
\textheight 235truemm % 226truemm
\textwidth 170truemm % 175truemm
\voffset -41truept % -14truept
\headsep 43truept % 18truept

\twocolumn
\columnsep 10truemm % 8truemm
%% end of A4 settings

%% This is for the US 8.5 x 11 paper size
%%\oddsidemargin  -0.31in
%%\evensidemargin -0.31in
%%
%%\topmargin 0truept
%%\headheight 0truept
%%\headsep 0truept
%%\footheight 0truept % for some reason this was left commented out for is2006
%%\footskip 0truept   % for some reason this was left commented out for is2006
%%\textheight 226truemm
%%\textwidth 175truemm
%%
%%\twocolumn
%%\columnsep 8truemm
%% end of 8.5x11 bit

\pagestyle{empty}
\def\ninept{\def\baselinestretch{0.95}\let\normalsize\small\normalsize}
\def\eightpt{\def\baselinestretch{0.95}\let\normalsize\footnotesize\normalsize}
% Make 9pt the default
\ninept



% adding titlebox
\newlength\titlebox
\setlength\titlebox{5cm}
\newcommand\anonname{
	\ifinterspeechfinal
	     \@name
    \else
         Anonymous submission to INTERSPEECH 2023
    \fi
}

\newcommand\anonaddress{
	\ifinterspeechfinal
	     \@address
    \fi
}

\newcommand\anonemail{
	\ifinterspeechfinal
	     \@email
    \fi
}


\def\maketitle{\par
 \begingroup
 \def\thefootnote{}
 \def\@makefnmark{\hbox
 to 0pt{$^{\@thefnmark}$\hss}}
 \if@twocolumn
 \twocolumn[\@maketitle]
 \else \newpage
 \global\@topnum\z@ \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\thefootnote{\arabic{footnote}}\gdef\@@savethanks{}%
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}


\def\@maketitle{\newpage
    {\vbox to \titlebox{
  \begin{center}
   {\large \bf \@title \par}
   \vskip 14pt {\large
     \textit{\anonname}
     \vskip 11pt
     \anonaddress}
     \vskip 3pt
     {\small\texttt{\anonemail}}
   \par\end{center}
 \par
 \thispagestyle{empty}
 \vskip 9pt}}
}

% \def\@maketitle{\newpage
%     {\vbox to \titlebox{
%   \begin{center}
%    {\large \bf \@title \par}
%    \vskip 1pt {\large
%      \textit{\anonname}
%      \vskip 1pt
%      \anonaddress}
%      \vskip 1pt
%      {\small\texttt{\anonemail}}
%    \par\end{center}
%  \par
%  \thispagestyle{empty}
%  \vskip 1pt}}
% }

\def\title#1{\gdef\@title{\Large{#1}}}
\def\name#1{\gdef\@name{#1\\}}
\def\address#1{\gdef\@address{#1\\}}
\def\email#1{\gdef\@email{#1}}
\gdef\@title{{Title of paper}}
\gdef\@name{{\em Name of author}\\}
\gdef\@address{Address - Line 1 \\
               Address - Line 2 \\
               Address - Line 3}
\gdef\@email{email@address}



\let\@@savethanks\thanks
\def\thanks#1{\gdef\thefootnote{}\@@savethanks{#1}}
\def\sthanks#1{\gdef\thefootnote{\fnsymbol{footnote}}\@@savethanks{#1}}

\def\@sect#1#2#3#4#5#6[#7]#8{
   \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname.\hskip 0.6em}
       \begingroup \ifnum #2=1\bf\centering
          {\interlinepenalty \@M
          \large{\@svsec #8}\par}\else\ifnum #2=2\bf
          \noindent{\interlinepenalty \@M \@svsec #8\par}\else
            \it
            \ifnum #2=3
            \noindent{\interlinepenalty \@M \@svsec #8\par}
            \else\@hangfrom{\hskip\parindent}{\interlinepenalty \@M
             \@svsec #8\par}\fi\fi\fi\endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\protect\numberline{\csname the#1\endcsname} #7}
     \@tempskipa #5\relax
     \@xsect{\@tempskipa}}

\def\abstract{\begin{center}
{\bf \large Abstract\vspace{-.5em}\vspace{2pt}}
\end{center}}
\def\endabstract{\par}

\def\copyrightnotice#1{\gdef\@copyrightnotice{#1}}\let\@copyrightnotice\relax
\def\toappear#1{\gdef\@toappear{#1}}\let\@toappear\relax

%%% Strings for the preprint titlepage footer:

\newif\if@preprint\@preprintfalse
\def\ds@preprint{\@preprinttrue}
\def\ps@preprint{\let\@mkboth\@gobbletwo\def\@oddhead{}
  \def\@oddfoot{\rlap{\@toappear}\hfil\thepage\hfil
    \llap{\@copyrightnotice}\gdef\@toappear{}\gdef\@copyrightnotice{}}}

\if@preprint\ps@preprint
\else\ps@empty\flushbottom\fi

\def\thebibliography#1{\section{References}\eightpt\list
 {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\flushbottom
%%%%% fancyheading included
\def\lhead{\@ifnextchar[{\@xlhead}{\@ylhead}}
\def\@xlhead[#1]#2{\gdef\@elhead{#1}\gdef\@olhead{#2}}
\def\@ylhead#1{\gdef\@elhead{#1}\gdef\@olhead{#1}}

\def\chead{\@ifnextchar[{\@xchead}{\@ychead}}
\def\@xchead[#1]#2{\gdef\@echead{#1}\gdef\@ochead{#2}}
\def\@ychead#1{\gdef\@echead{#1}\gdef\@ochead{#1}}

\def\rhead{\@ifnextchar[{\@xrhead}{\@yrhead}}
\def\@xrhead[#1]#2{\gdef\@erhead{#1}\gdef\@orhead{#2}}
\def\@yrhead#1{\gdef\@erhead{#1}\gdef\@orhead{#1}}

\def\lfoot{\@ifnextchar[{\@xlfoot}{\@ylfoot}}
\def\@xlfoot[#1]#2{\gdef\@elfoot{#1}\gdef\@olfoot{#2}}
\def\@ylfoot#1{\gdef\@elfoot{#1}\gdef\@olfoot{#1}}

\def\cfoot{\@ifnextchar[{\@xcfoot}{\@ycfoot}}
\def\@xcfoot[#1]#2{\gdef\@ecfoot{#1}\gdef\@ocfoot{#2}}
\def\@ycfoot#1{\gdef\@ecfoot{#1}\gdef\@ocfoot{#1}}

\def\rfoot{\@ifnextchar[{\@xrfoot}{\@yrfoot}}
\def\@xrfoot[#1]#2{\gdef\@erfoot{#1}\gdef\@orfoot{#2}}
\def\@yrfoot#1{\gdef\@erfoot{#1}\gdef\@orfoot{#1}}

\newdimen\headrulewidth
\newdimen\footrulewidth
\newdimen\plainheadrulewidth
\newdimen\plainfootrulewidth
\newdimen\headwidth
\newif\if@fancyplain
\def\fancyplain#1#2{\if@fancyplain#1\else#2\fi}

% Command to reset various things in the headers:
% a.o.  single spacing (taken from setspace.sty)
% and the catcode of ^^M (so that epsf files in the header work if a
% verbatim crosses a page boundary)
\def\fancy@reset{\restorecr
 \def\baselinestretch{1}%
 \ifx\undefined\@newbaseline% NFSS not present; 2.09 or 2e
  \ifx\@currsize\normalsize\@normalsize\else\@currsize\fi%
 \else% NFSS (2.09) present
  \@newbaseline%
 \fi}

% Initialization of the head and foot text.

\headrulewidth 0.4pt
\footrulewidth\z@
\plainheadrulewidth\z@
\plainfootrulewidth\z@

\lhead[\fancyplain{}{\sl\rightmark}]{\fancyplain{}{\sl\leftmark}}
%  i.e. empty on ``plain'' pages, \rightmark on even, \leftmark on odd pages
\chead{}
%\rhead[\fancyplain{}{\sl\leftmark}]{\fancyplain{}{\sl\rightmark}}
%  i.e. empty on ``plain'' pages, \leftmark on even, \rightmark on odd pages
\lfoot{}
\cfoot{}
\rfoot{}

% Put together a header or footer given the left, center and
% right text, fillers at left and right and a rule.
% The \lap commands put the text into an hbox of zero size,
% so overlapping text does not generate an errormessage.

\def\@fancyhead#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset\vbox{\hbox
{\rlap{\parbox[b]{\headwidth}{\raggedright#2\strut}}\hfill
\parbox[b]{\headwidth}{\centering#3\strut}\hfill
\llap{\parbox[b]{\headwidth}{\raggedleft#4\strut}}}\headrule}}#5}


\def\@fancyfoot#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset\vbox{\footrule
\hbox{\rlap{\parbox[t]{\headwidth}{\raggedright#2\strut}}\hfill
\parbox[t]{\headwidth}{\centering#3\strut}\hfill
\llap{\parbox[t]{\headwidth}{\raggedleft#4\strut}}}}}#5}

\def\headrule{{\if@fancyplain\let\headrulewidth\plainheadrulewidth\fi
\hrule\@height\headrulewidth\@width\headwidth \vskip-\headrulewidth}}

\def\footrule{{\if@fancyplain\let\footrulewidth\plainfootrulewidth\fi
\vskip-0.3\normalbaselineskip\vskip-\footrulewidth
\hrule\@width\headwidth\@height\footrulewidth\vskip0.3\normalbaselineskip}}

\def\ps@fancy{%
\@ifundefined{@chapapp}{\let\@chapapp\chaptername}{}%for amsbook
\@ifundefined{chapter}{\def\sectionmark##1{\markboth
{\uppercase{\ifnum \c@secnumdepth>\z@
 \thesection\hskip 1em\relax \fi ##1}}{}}%
\def\subsectionmark##1{\markright {\ifnum \c@secnumdepth >\@ne
 \thesubsection\hskip 1em\relax \fi ##1}}}%
{\def\chaptermark##1{\markboth {\uppercase{\ifnum \c@secnumdepth>\m@ne
 \@chapapp\ \thechapter. \ \fi ##1}}{}}
\def\sectionmark##1{\markright{\uppercase{\ifnum \c@secnumdepth >\z@
 \thesection. \ \fi ##1}}}}%
\csname ps@headings\endcsname % use \ps@headings defaults if they exist
\ps@@fancy
\gdef\ps@fancy{\@fancyplainfalse\ps@@fancy}%
\headwidth\textwidth}
\def\ps@fancyplain{\ps@fancy \let\ps@plain\ps@plain@fancy}
\def\ps@plain@fancy{\@fancyplaintrue\ps@@fancy}
\def\ps@@fancy{%
\def\@mkboth{\protect\markboth}%
\def\@oddhead{\@fancyhead\@lodd\@olhead\@ochead\@orhead\@rodd}%
\def\@oddfoot{\@fancyfoot\@lodd\@olfoot\@ocfoot\@orfoot\@rodd}%
\def\@evenhead{\@fancyhead\@rodd\@elhead\@echead\@erhead\@lodd}%
\def\@evenfoot{\@fancyfoot\@rodd\@elfoot\@ecfoot\@erfoot\@lodd}%
}
\def\@lodd{\if@reversemargin\hss\else\relax\fi}
\def\@rodd{\if@reversemargin\relax\else\hss\fi}

\let\latex@makecol\@makecol
\def\@makecol{\let\topfloat\@toplist\let\botfloat\@botlist\latex@makecol}
\def\iftopfloat#1#2{\ifx\topfloat\empty #2\else #1\fi}
\def\ifbotfloat#1#2{\ifx\botfloat\empty #2\else #1\fi}
\def\iffloatpage#1#2{\if@fcolmade #1\else #2\fi}


